NeoRL-2: Near Real-World Benchmarks for Offline Reinforcement Learning with Extended Realistic Scenarios

Offline reinforcement learning (RL) aims to learn from historical data without requiring (costly) access to the environment. To facilitate offline RL research, we previously introduced NeoRL, which highlighted that datasets from real-world tasks are often conservative and limited. With years of experience applying offline RL to various domains, we have identified additional real-world challenges. These include extremely conservative data distributions produced by deployed control systems, delayed action effects caused by high-latency transitions, external factors arising from the uncontrollable variance of transitions, and global safety constraints that are difficult to evaluate during the decision-making process. These challenges are underrepresented in previous benchmarks but frequently occur in real-world tasks. To address this, we constructed the extended Near Real-World Offline RL Benchmark (NeoRL-2), which consists of 7 datasets from 7 simulated tasks along with their corresponding evaluation simulators. Benchmarking results from state-of-the-art offline RL approaches demonstrate that current methods often struggle to outperform the data-collection behavior policy, highlighting the need for more effective methods. We hope NeoRL-2 will accelerate the development of reinforcement learning algorithms for real-world applications. The benchmark project page is available at https://github.com/polixir/NeoRL2.

==> sec_text/conclusion.tex <==
\section{Conclusion}
Offline RL aims to learn from historical data, eliminating the need for new data collection in real-world environments. To evaluate the effectiveness of offline RL algorithms, various benchmark suites have been proposed. However, existing benchmarks often fail to fully capture the critical characteristics of real-world tasks. To address this, we introduce NeoRL-2, a benchmark suite that encompasses tasks in robotics, aerial vehicles, industrial pipelines, nuclear fusion, and the medical fields. These tasks incorporate features such as delays, external factors, and constraints, making NeoRL-2 more representative of real world scenarios. We employ a deterministic method for sampling and restrict the number of samples, aligning with realistic task settings. Additionally, in certain specialized scenarios, we incorporate the classic PID controller as a data sampling method. We tested SOTA offline RL algorithms using NeoRL-2 and analyzed the results. Our experimental results indicate that, in most tasks, these algorithms do not significantly outperform the policies used for data collection. Through this work, we aim to promote a closer integration of offline RL algorithm research with real-world application, facilitating the practical implementation of RL in real-world scenarios.

\tzl{NeoRL-2 is designed to provide a range of easy-to-use simulation environments for evaluating offline reinforcement learning algorithms, however, there are still gaps between the benchmarking results and the real-world performances of current offline RL algorithms. The simulation environments still cannot fully replicate the complexity of real-world tasks, especially when the transition of some real-world tasks is unclear. This is also a common issue faced by the offline RL community, and we believe NeoRL-2 will facilitate the development of both the future benchmark tasks and offline algorithms.}

==> sec_text/experiments.tex <==
\section{Experiments}

\subsection{Comparing Methods}
We validated the following methods in the tasks of NeoRL-2.

\subsubsection{Baseline}
{\bf Expert Policy.} Specifically, we use the soft actor-critic (SAC)~\citep{sac2018} algorithm to perform online policy improvement for each environment in NeoRL-2. The model achieving the highest score will be saved. It is important to note that the highest-scoring policy obtained by SAC represents a good policy, but not necessarily the optimal one. \textbf{In normalization of data scores (0-100), the scores given by expert policies are used as the maximum bound.}

{\bf Random Policy.} We employ uniform random sampling to generate actions within the action space of each environment. The random policy is generally considered a poor policy, often demonstrating terrible performance. \textbf{The performance of this policy in the environment is typically used as the minimum bound for the normalization of data scores (0-100).}

{\bf Behavior Policy.} This approach involves preserving sub-optimal policies generated during the SAC-training of expert policies. In the real world, most offline data collection does not achieve optimal policy performance, resulting in offline datasets. If some environments already had optimal policies, there would be no need to apply RL for performance improvement. Thus, we compile datasets from the policies saved during SAC training and record the average return value of the trajectories in these datasets. Note that the dataset for DMSD is collected using a PID policy.


\subsubsection{Model-Free Methods}
To establish a comprehensive benchmark, we include several representative algorithms for offline policy improvement. These include the Behavior Cloning (BC) method, which uses supervised learning to replicate the policies from the data. We also implement offline RL methods such as CQL \citep{2020cql}, EDAC \citep{2021edac}, MCQ \citep{2022mcq}, and TD3BC \citep{2021td3bc}. All Methods implementations can be viewed at \href{https://github.com/polixir/OfflineRL}{Github}\footnote{https://github.com/polixir/OfflineRL}.


\begin{itemize}[itemsep=0pt,topsep=0pt,parsep=0pt,leftmargin=*]
    \item \emph{CQL}~\citep{2020cql}.
    Conservative $Q$-Learning (CQL) method prevents overestimation of the state-action value function $Q$ by especially penalizing out-of-distribution (OOD) data points. By obtaining a conservative $Q$ function, CQL minimizes the difference between the current $Q$-values and the true values in the data, while training the policy by maximizing the $Q$ function. This approach, applied within the SAC framework, effectively mitigates the issue of $Q$-value overestimation, resulting in a more reliable offline policy improvement algorithm.
    
    \item \emph{EDAC}~\citep{2021edac}. Ensemble-Diversifying Actor-Critic (EDAC) method builds upon the SAC algorithm by utilizing the clipped $Q$-learning method, commonly used in online RL, to effectively penalize OOD data points. The clipped $Q$-learning method computes a pessimistic estimate by choosing the minimum of $Q$-value. Additionally, EDAC significantly enhances the algorithm's effectiveness by increasing the number of $Q$-networks, which is also proved beneficial in various actor-critic algorithms. 
    By incorporating Ensemble Gradient Diversification, EDAC effectively reduces the number of $Q$-networks while maintaining, and even surpassing, the effectiveness of SOTA algorithms.

    \item \emph{MCQ}~\citep{2022mcq}. Mildly Conservative $Q$-learning (MCQ) method aims to reduce the overestimation of the $Q$ function, particularly by maintaining conservatism for OOD actions. When adding a penalty term for OOD data, the value of this penalty is based on assigning appropriate scores to OOD data within the constructed $Q$-network, rather than simply increasing the penalty strength. Experimental results show that this conservative approach does not significantly cause overestimation in the $Q$ network and achieves commendable performance.
    
    \item \emph{TD3BC}~\citep{2021td3bc}. TD3BC makes slight modifications to existing RL algorithms but achieves significant performance improvements. It modifies the policy gradient component of the Twin Delayed Deep Deterministic Policy Gradient (TD3) algorithm \citep{2018Fujimoto}. For objective function, the state-action value function result subtracts the Mean Squared Error (MSE) between the current policy network output and the action from the dataset. Essentially, TD3BC adds a BC regularization term to the standard policy update of TD3 to encourage the policy to favor actions present in the training dataset.
    
\end{itemize}

\subsubsection{ Model-Based Methods}
The advantages of model-based offline RL over model-free methods include higher data utilization efficiency, faster convergence speed, and great explainability. By utilizing offline data for environment model training, model-based methods can effectively make use of the available data. We employ model-based RL methods, including MOPO \citep{yu2020mopo}, COMBO \citep{2021combo}, RAMBO \citep{2022rambo}, and Mobile \citep{2023mobile}. These methods construct a dynamic model from the data and use this model to enhance policies.

\begin{itemize}[itemsep=0pt,topsep=0pt,parsep=0pt,leftmargin=*]
    \item \emph{MOPO}~\citep{yu2020mopo}. Model-based Offline Policy Optimization focuses one the distribution shift problem between the trained dynamic model and the real environment in model-based RL. To mitigate this issue, during subsequent policy learning, the rewards obtained from interactions between the policy network and the model are augmented with a penalty that accounts for the discrepancy between the model and the real data. This ensures that the policy, when making action choices, considers the extent of deviation from real environment transitions. By aligning the policy as closely as possible with the transition dynamics in the data, MOPO aims to optimize the policy effectively.
    \item \emph{COMBO}~\citep{2021combo}. 
    Conservative Offline Model-Based Policy Optimization extends MOPO by additionally addressing potential inaccuracies in calculating the discrepancy between the model and the real data, as well as poor performance in some scenarios. During the training of the value network, COMBO incorporates both offline datasets and model-generated data, introducing an additional regularization term to generated out-of-support state-action pairs. This approach enables a conservative estimate of the value function without the need to directly measure the error between generated data and offline data, thereby enhancing the robustness and performance of the algorithm.
    \item \emph{RAMBO}~\citep{2022rambo}. Robust Adversarial Model-Based Offline RL constructs the dynamic model using the BC method. Based on that, RAMBO performs model-based policy improvement, primarily using the SAC algorithm structure. Notably, RAMBO samples from a buffer that combines training data with trajectory data generated by the model. During each update cycle, the model also undergoes updates. By utilizing maximum likelihood estimates to adjust the model, RAMBO influences the loss function. This approach ensures that the model continuously approximates the environment transitions present in the training data throughout the policy training process.
    \item \emph{Mobile}~\citep{2023mobile}. To ensure conservatism in its usage, Mobile incorporates Model Bellman Inconsistency as a measure of uncertainty to assess the discrepancy between generated data and offline data. This metric allows for quantitative analysis of the inconsistency of Bellman estimations produced by the ensemble of dynamic models. In regions where there is abundant offline data, Bellman estimations typically exhibit small errors and low discrepancies between estimations. However, in regions with rare data, there is a higher inconsistency between Bellman estimations. Mobile addresses actions with poor consistency of Bellman estimations by applying larger penalties, further ensuring that the policy avoids risky actions in such regions.
    
    % VariBAD (Variational Bayes for Adaptive Deep RL) is also a meta-RL method that uses variational inference to enable fast adaptation to new tasks. It employs a Bayesian approach to meta-learning, inferring task-specific posterior distributions over the parameters of the policy and value function. Specifically, it first learns an RNN variational auto-encoder to extract the sequential features of the dynamics or tasks. The policy then receives the current state and the output of the context encoder to make adaptive decisions.
\end{itemize}

\subsection{Benchmarking Results}
\label{sec.bm_result}

\begin{figure}[htbp] 
\centering 
\includegraphics[width=1\textwidth]{figures/resultshist.png} 
\caption{The baseline algorithm normalized scores over seven environments comparing with that of offline data.}
\label{fig.resultshist} 
\end{figure}
As there are no very stable and consistent offline policy evaluation methods~\cite{OffPolicyEval,qinr2022neorl}, we only conduct online policy evaluation. We run each configuration of the hyperparameters with 3 random seeds and choose the policy at the final training stage to conduct the online test. We report the results from the best hyperparameter across 3 seeds and the 3 seeds are the same for all the algorithms.
Figure \ref{fig.resultshist} illustrates the normalized scores obtained by the baseline algorithm, with each color and symbol representing a different baseline algorithm as indicated in the legend. This visualization, derived from Table \ref{table.algo_final}, offers an intuitive overview of the performance of tuned hyper-parameters that yield the highest mean score among the current algorithms. The performance of each algorithm on specific tasks is computed using three random seeds, and their standard errors are depicted with error bars. From an environmental perspective, the performance of almost all baseline algorithms surpasses the scores in the offline data in the RandomFrictionHopper and DMSD environments. Model-based algorithms demonstrate lower stability compared to model-free algorithms, particularly evident in the RocketRecovery, Fusion, and SafetyHalfCheetah tasks, where MOPO and RAMBO exhibit larger error bars. This highlights the heightened sensitivity of MOPO and RAMBO algorithms to random seed selection in these tasks, while other algorithms showcase smaller error bars, indicating better stability. In terms of scores, no algorithm surpasses 95 in any task \footnote{95 of normalized score can be treated as having solved the task.}. The TD3BC algorithm achieves the highest score of 81.95 points in the Pipeline task but falls short of 95 points. Consequently, we have yet to identify any algorithm capable of successfully solving the tasks in NeoRL-2, and there has been no significant improvement in scores compared to those in the data.

\begin{table}[ht]
\centering
\small
\setlength{\tabcolsep}{6pt} 
\renewcommand{\arraystretch}{1.5} 
\caption{The parameter configuration that achieves the highest score in the baseline algorithm over all 7 environments. $\pm$ denotes standard error over three random seeds.}
\label{table.algo_final}
\resizebox{1\textwidth}{!}{
\begin{tabular}{l|c r@{~$\pm$~}l r@{~$\pm$~}l r@{~$\pm$~}l r@{~$\pm$~}l r@{~$\pm$~}l r@{~$\pm$~}l r@{~$\pm$~}l r@{~$\pm$~}l r@{~$\pm$~}l}
\toprule
& \textbf{Data} & \multicolumn{2}{c}{\textbf{BC}} & \multicolumn{2}{c}{\textbf{CQL}} & \multicolumn{2}{c}{\textbf{EDAC}} & \multicolumn{2}{c}{\textbf{MCQ}} & \multicolumn{2}{c}{\textbf{TD3BC}} & \multicolumn{2}{c}{\textbf{MOPO}} & \multicolumn{2}{c}{\textbf{COMBO}} & \multicolumn{2}{c}{\textbf{RAMBO}} & \multicolumn{2}{c}{\textbf{MOBILE}} \\
\midrule
\textbf{Pipeline} & 69.25 & 68.61 & 13.42 & 81.08 & 8.25 & 72.88 & 4.64 & 49.7 & 7.39 & \bf{81.95} & \bf{7.46} & -26.33 & 92.65 & 55.50 & 4.28 & 24.06 & 74.39 & 65.51 & 4.05 \\
\textbf{Simglucose} & 73.87 & \bf{75.07} & \bf{0.71} & 10.99 & 3.35 & 8.11 & 0.31 & 29.57 & 5.65 & 74.21 & 0.38 & 34.64 & 28.13 & 23.18 & 2.47 & 10.8 & 0.86 & 9.29 & 0.17 \\
\textbf{RocketRecovery} & 75.27 & 72.75 & 2.53 & 74.32 & 1.44 & 65.65 & 9.81 & 76.46 & 0.81 & \bf{79.74} & \bf{0.91} & -27.66 & 105.61 & 74.66 & 0.70 & -44.21 & 263.00 & 43.71 & 17.53 \\
\textbf{RandomFrictionHopper} & 28.73 & 28.03 & 0.35 & 32.96 & 1.23 & 34.69 & 1.29 & 31.74 & 1.25 & 29.51 & 0.66 & 32.48 & 5.79 & 34.08 & 4.74 & 29.62 & 7.15 & \bf{35.12} & \bf{0.47} \\
\textbf{DMSD} & 56.64 & 65.09 & 1.64 & 70.24 & 1.12 & \bf{78.65} & \bf{2.30} & 77.75 & 1.16 & 60.01 & 0.79 & 68.23 & 0.65 & 68.33 & 0.41 & 76.22 & 1.92 & 64.36 & 0.78 \\
\textbf{Fusion} & 48.75 & 55.24 & 0.30 & 55.86 & 1.89 & 58.00 & 0.72 & 49.70 & 1.05 & 54.64 & 0.82 & -11.60 & 22.20 & 55.48 & 0.28 & \bf{59.63} & \bf{4.99} & 5.02 & 7.05 \\
\textbf{SafetyHalfCheetah} & \bf{73.56} & 70.16 & 0.38 & 71.18 & 0.61 & 53.11 & 11.14 & 54.65 & 4.32 & 68.58 & 0.39 & 23.71 & 24.28 & 57.79 & 13.27 & -422.43 & 307.49 & 8.68 & 3.93 \\
\bottomrule
\end{tabular}
}
\end{table}
Table \ref{table.algo_final} presents the highest scores of all baseline algorithms with tuned hyper-parameters in the NeoRL-2 tasks, along with the standard errors computed from three random seeds. From Table~\ref{table.algo_final}, it is evident that in the SafetyHalfCheetah task, none of the algorithms exceed the scores in the offline data, with RAMBO exhibiting particularly high standard errors, indicating significant instability. The most notable improvement in scores is observed in the DMSD task, where the EDAC algorithm's performance increases to 78.56, representing an improvement of about 22 scores.

% \begin{figure}[htbp]
%     \centering
%     \begin{subfigure}{.5\textwidth}
%         \centering
%         \includegraphics[width=0.95\textwidth]{figures/resultrate.png}
%         \caption{The proportion of a baseline algorithm whose scores exceeding the data scores.}
%         \label{fig.resultrate}
%     \end{subfigure}%
%     \begin{subfigure}{.5\textwidth}
%         \centering
%         \begin{tabular}{l|cccc}
%         \toprule
%          & +0 & +3 & +5 & +10 \\
%         \midrule
%         BC & 3 & 2 & 2 & 0 \\
%         CQL & 4 & 4 & 3 & 2 \\
%         EDAC & 4 & 4 & 3 & 1 \\
%         MCQ & 4 & 2 & 1 & 1 \\
%         TD3BC & 6 & 4 & 2 & 1 \\
%         MOPO & 2 & 2 & 1 & 1 \\
%         COMBO & 3 & 3 & 3 & 1 \\
%         RAMBO & 3 & 2 & 2 & 2 \\
%         MOBILE & 2 & 2 & 2 & 0 \\
%         \bottomrule
%         \end{tabular}
%         \caption{The specific number of tasks that an algorithm surpassing data scores.}
%         \label{table.scoresover}
%     \end{subfigure}
% \end{figure}

\begin{figure}[h]
    \centering
    \begin{minipage}[b]{0.45\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/resultrate.png} % 插入图片，修改为你的图片路径
        \caption{The proportion of a baseline algorithm whose scores exceeding the data scores.}
        \label{fig.resultrate}
    \end{minipage}
    \hfill
    \begin{minipage}[b]{0.45\textwidth}
        \centering
        \begin{tabular}{l|cccc}
        \toprule
         & +0 & +3 & +5 & +10 \\
        \midrule
        BC & 3 & 2 & 2 & 0 \\
        CQL & 4 & 4 & 3 & 2 \\
        EDAC & 4 & 4 & 3 & 1 \\
        MCQ & 4 & 2 & 1 & 1 \\
        TD3BC & 6 & 4 & 2 & 1 \\
        MOPO & 2 & 2 & 1 & 1 \\
        COMBO & 3 & 3 & 3 & 1 \\
        RAMBO & 3 & 2 & 2 & 2 \\
        MOBILE & 2 & 2 & 2 & 0 \\
        \bottomrule
        \end{tabular}
        \tabcaption{The specific number of tasks that an algorithm surpassing data scores.}
        \label{table.scoresover}
    \end{minipage}
\end{figure}


Figure \ref{fig.resultrate} compares the proportion of baseline algorithms that exceed data scores in seven tasks. The results show that the TD3BC algorithm surpasses data scores in more than 80\% of the tasks. Additionally, the proportion of successes is higher for model-free algorithms compared to model-based ones. It is worth mentioning that the proportion calculated here is based on the results from Table \ref{table.algo_final}, where any algorithm's score surpassing the data score is counted as a successful improvement. This approach may result in cases where the scores are close but the improvement is not significant.



% \begin{table}[ht]
% \centering
% \small
% \caption{The specific number of tasks that an algorithm surpassing data scores.}
% \label{table.scoresover}
% \resizebox{0.4\textwidth}{!}{
% \begin{tabular}{l|cccc}
% \toprule
%  & +0 & +3 & +5 & +10 \\
% \midrule
% \text{BC} & 3 & 2 & 2 & 0 \\
% \text{CQL} & 4 & 4 & 3 & 2 \\
% \text{EDAC} & 4 & 4 & 3 & 1 \\
% \text{MCQ} & 4 & 2 & 1 & 1 \\
% \text{TD3BC} & 6 & 4 & 2 & 1 \\
% \text{MOPO} & 2 & 2 & 1 & 1 \\
% \text{COMBO} & 3 & 3 & 3 & 1 \\
% \text{RAMBO} & 3 & 2 & 2 & 2 \\
% \text{MOBILE} & 2 & 2 & 2 & 0 \\
% \bottomrule
% \end{tabular}
% }
% \end{table}

Table \ref{table.scoresover} specifically lists the number of times each baseline algorithm exceeds the scores in the data. Here, +0, +3, +5, and +10 represent the thresholds for exceeding the scores in the data. For example, +10 means that the algorithm's score exceeds the data score by more than 10 points. With these results, we can gain a more intuitive understanding of the degree of improvement for each algorithm. From the results, RAMBO and CQL achieved a 10-score improvement in two out of seven tasks. However, none of the algorithms can achieve a 5-score improvement in more than half of the tasks. These findings suggest that current baseline algorithms have not significantly improved performance in the NeoRL-2 tasks. While there may be improvements in some tasks, we have not observed any algorithm that can achieve a 5-point improvement in most tasks. This indirectly indicates that in the tasks where these SOTA algorithms achieve significant performance improvements, the tasks are relatively simple. Once these tasks are replaced by the NeoRL-2 tasks, which are closer to the real world, the performance of these algorithms is far from the performance they claim.







==> sec_text/intro.tex <==
\section{Introduction}
% Give an introduction for offline RL, the current reality gap between previous benchmarks and the realistic scenarios (the necessity of NeoRL 2.0).

Reinforcement learning (RL) learns the optimal policy through trial-and-error in the environment, demonstrating excellent performance in various fields. From traditional game domains such as Go~\citep{silver2016alphago,silver2017alphazero} and Atari games~\citep{mnih2015human} to complex real-world tasks like recommender systems~\citep{2019VirtualTaobao} and sciences, such as Tokamak control~\citep{2022tokamak}, the application scope of RL continues to expand. However, when a fast and low-cost simulator is absent, conventional RL is hard to be applied~\citep{2021Gabriel}. This necessitates the need for offline RL~\citep{batchRL}. Offline RL learns a policy from static historical data, which alleviates the costly interaction with the environment. 

% However, there are indeed challenges when applying RL methods to real-world scenarios. Firstly, operating costs in real environments are often high. Some tasks may require expensive hardware infrastructure and human resources, which makes trial-and-error and policy optimization in practical environments costly and unsafe. For example, in the automated production lines of factories, reinforcement learning strategies may take unforeseen actions during the implementation process, which could pose risks to personnel or equipment.

% Additionally, RL typically requires extensive interaction and trial-and-error processes to learn effective policies, while in certain real-world application scenarios, the experimentation cycles can be lengthy, resulting in low time efficiency. For instance, in the field of drug development, clinical trials involve prolonged observation and evaluation, limiting the speed and efficiency of applying RL methods in practical environments.

% Why this paragraph here. This para tends to state that the data issue in the offline setting, while the next para turns to the solution of offline RL. This is weird.
% Lastly, acquiring large amounts of high-quality training data can be challenging in certain application scenarios. For example, in safety-sensitive domains like nuclear energy or aerospace, obtaining data from real environments may be restricted, leading to data scarcity issues that constrain the feasibility and effectiveness of RL methods in practical environments.

% These aforementioned challenges necessitate the search for solutions, such as offline reinforcement learning. Offline reinforcement learning is considered a potential solution that can alleviate these problems to some extent. It leverages existing historical data for policy learning and optimization, avoiding direct interaction with the environment. In practical applications, the available historical dataset is often extensive, and offline reinforcement learning aims to maximize the utilization of this data by treating policies as decision engines, thereby avoiding the series of issues associated with online reinforcement learning that require environment interaction.

% However, existing online RL benchmarks are primarily designed for online learning algorithms and tasks, with a focus on maximizing rewards, which fails to fully capture the heterogeneity and complexity of real-world data. These benchmarks are not effectively applicable to the specific requirements of offline learning. Therefore, it is necessary to design specialized benchmarks and datasets specifically tailored for offline reinforcement learning algorithms in order to accurately evaluate their performance and compare different approaches.

Existing benchmarks for offline RL, such as D4RL~\citep{D4RL, 2021justin} and RL Unplugged~\citep{RLunplugged}, have significantly contributed to the development of offline RL. These benchmarks often focus on using historical data collected with different policies as offline datasets, and the tasks themselves are common benchmark tasks for online RL that may not fully capture the complexity of real-world application scenarios. For example, in real industrial systems, observations and rewards may contain significant delays due to sensor sampling and signal transmission \citep{1999Tan}. The data-collecting policies in real-world scenarios often utilize samples obtained from the operational control system without exploration. Real-world task scenarios are often not closed systems and are influenced by many external factors. Besides, the amount of historical data in the real world is small. The NeoRL~\citep{qinr2022neorl} benchmark has included conservative and limited datasets to reflect these two common properties in real-world datasets. Although NeoRL provides simulated domains from real-world tasks, such as industrial control, and urban energy management, some critical challenges have not been contained. \tzl{In the real-world tasks we have experienced, there are effects of time delay, external factors, and safety constraints, which are also widely present in industry. For example, in a water treatment plant, the physical distance between pumps results in noticeable time delay effects for actions. There are delayed action effects when the environment has high latency and uncontrollable external factors that may affect the policy. When controlling drone flights, unpredictable winds in the environment can cause significantly different outcomes for the same control inputs, and these external factors are not influenced by the policy. Safety constraints are also prevalent in industrial environments; certain equipment must operate under specific conditions (e.g., temperature, speed), which restricts the action space. The operating policy should obey global safety constraints such that the offline datasets do not contain any unsafe behaviors. Thus, the offline algorithm has to learn a better and safer policy without knowing unsafe data.}

From these real-world scenarios, we have summarized some common characteristics: {\bf time delay}, {\bf external factors}, {\bf policy constraints}, {\bf data collected based on traditional control methods}, and {\bf limitations on data}. To further bridge the gap \tzl{and provide as many challenges as possible across different real-world scenarios, we extend NeoRL by proposing NeoRL-2. In NeoRL-2, we incorporated the above five common characteristics into seven tasks, making the benchmarks obtained from these tasks close to real-world scenarios.} It is important to note that we cannot directly use real business data in our benchmark due to infeasible real-world evaluation as well as data privacy. Thus, we purposely construct simulators for collecting datasets and evaluating policies. These simulators are not necessarily very sophisticated and realistic, but should exhibit important practical challenges for developing advanced algorithms.

NeoRL-2 includes new task scenarios that better reflect real-world task properties and includes traditional control methods as the data-collecting method. In summary, our contributions are as follows.

\begin{enumerate}[itemsep=0pt,topsep=0pt,parsep=0pt,leftmargin=*]
\item Tasks in NeoRL-2 cover a wider range of application domains, including robotics, aircraft, industrial pipelines, controllable nuclear fusion, healthcare, etc., encompassing key features such as delays, external factors, and safety constraints.

\item The data-collecting method in NeoRL-2 better aligns with real-world scenarios, employing deterministic methods for sampling. In some specific tasks, classical feedback controllers, such as Proportional-Integral-Derivative (PID) controller~\cite{johnson2005pid}, are introduced.

\item We conducted experiments on these tasks using state-of-the-art (SOTA) offline RL algorithms and found that in most tasks, the trained policy of the current offline RL algorithms did not significantly outperform the behavior policy.
\end{enumerate}

By extending near real-world tasks in NeoRL-2, we hope that the development and implementation of RL in real-world scenarios can take into account these challenges and tackle more realistic domains.





==> sec_text/neorlintro.tex <==
\section{NeoRL-2 Tasks and Datasets}
In this section, we will provide a brief overview of all tasks included in NeoRL-2. Each task comprises a corresponding environment and dataset composition, with the dataset used for training policies and the environment used for policy testing.

\subsection{Tasks}

Next, we will provide a brief overview of the 7 tasks included in NeoRL-2. These tasks consist of a pipeline flow task and a human blood glucose concentration simulator, both of which exhibit significant time delay characteristics. Additionally, we have developed two additional environments: Rocket Recovery and Random Friction Hopper. In these environments, there are external factors that need to be included as part of the observations. To facilitate data collection using the PID control method, we constructed the Double Mass Spring Damper (DMSD) environment. Furthermore, the Safety Halfcheetah is a simulated task that imposes action constraints to ensure actions remain within a safe range. Finally, we have the Fusion environment, which represents the type of tasks in the real world where collecting offline data is extremely costly. In these tasks, the collection of offline data is particularly expensive, making the Fusion environment a representative example of such tasks.

{\bf Pipeline.} The Pipeline simulator models the flow of water through a 100-meter-long pipeline with a fixed velocity. The controller's objective is to regulate the flow rate by adjusting the inlet water gate. The simulation runs for 1000 time steps, with the target flow rate at the outlet influenced by an external policy and randomly selected from the set [50, 80, 110, 140]. At each time step, there is a 0.3\% probability of changing the target flow rate, averaging three changes per simulation.

{\bf Simglucose.}
The Simglucose simulator \citep{man2014uva} accurately simulates a diabetic patient's intricate blood glucose concentration variations throughout a day, starting at 8 a.m. The comprehensive simulator encompasses patient simulation, scenario simulation, sensor simulation, and insulin pump simulation. The patient randomly consumes meals and medication, with their effects gradually manifesting over time. The policy's primary objective is to safely control the medication regimen, ensuring that blood glucose levels remain within a desired range while accounting for the delayed effects of medication. This environment proves invaluable in optimizing and refining diabetes treatment strategies.


{\bf RocketRecovery.} The RocketRecovery simulator modifies the lunar\_lander\footnote{https://www.gymlibrary.dev/environments/box2d/lunar\_lander/} environment from Gym, incorporating wind force as an external factor. The task's objective is to land the rocket safely and as close to the target as possible, while maintaining safe angles and velocities. This environment presents a classic rocket trajectory optimization problem.

{\bf RandomFrictionHopper.} The RandomFrictionHopper simulator is a variation of the classic Hopper task, where a single-legged robot jumps and moves by controlling its leg actions. Each initialization sets a random ground friction coefficient in the range [1.5, 2.5], which is included as an extended dimension of the state observation. This variation introduces variability in the task's dynamics.

{\bf DMSD.} The Double Mass Spring Damper simulator involves two blocks with masses connected by springs and dampers. The task requires applying forces to control and stabilize the blocks at target positions. Notably, the interconnected springs and dampers mean that applying force to one block affects the other one. Each step in the simulation corresponds to 0.2 seconds in the real world, with a 100-step limit before automatic truncation.

{\bf SafetyHalfCheetah.} The SafetyHalfCheetah simulator is a variant of the HalfCheetah task, emphasizing safe high-speed running. In this task, the robot must sprint at maximum speed while ensuring its motion remains within safe limits to prevent accidents and damage. This task balances speed and safety, simulating real-world scenarios that require high-speed but safe robotic movement. Once the agent breaks the constraint, the environment will terminate and give a large negative score.

{\bf Fusion.} The Fusion simulator simulates the control of a Tokamak device for nuclear fusion. The objective is to control the Tokamak device solely based on observational states and attempt to stabilize the system at a target position during operation. However, the cost of conducting Tokamak device experiments in the real world is particularly high, making collected offline data in this environment valuable and data sparse. Due to the complexity of numerical simulations of Tokamak devices and the inherent error between numerical simulations and real device states, an LSTM neural network model has been utilized to "clone" the Tokamak device based on collected data \citep{Seo_2021}. We treat the "clone" model as a simulator of the Fusion task.


\begin{table}[ht]
\centering
\small
\caption{The table comparing the characteristics of each task.}
\label{table.taskcharacter}
\resizebox{1\textwidth}{!}{
\begin{tabular}{l|ccccc}
\toprule
& \multirow{3}{*}{Delay} & \multirow{3}{*}{External factors} & \multirow{3}{*}{\parbox{1.5cm}{\centering Constrained \\ control policies}} & \multirow{3}{*}{\parbox{2.5cm}{\centering Data from traditional \\ control methods}} & \multirow{3}{*}{\parbox{2.5cm} {Limitations on \\data availability}} \\
\\
\\

\midrule
Pipeline & $\checkmark$ & -- & -- & -- & -- \\
Simglucose & $\checkmark$  & $\checkmark$  & -- & -- & --  \\
RocketRecovery & -- &  $\checkmark$ & -- & -- & $\checkmark$ \\
RandomFrictionHopper & -- & $\checkmark$ & -- & -- & --\\
DMSD & -- & -- & -- & $\checkmark$ & -- \\
Fusion & -- & -- & -- &  -- & $\checkmark$ \\
SafetyHalfCheetah & -- & -- & $\checkmark$ & -- & $\checkmark$ \\
\bottomrule
\end{tabular}
}
\end{table}

Table \ref{table.taskcharacter} marks the characteristics possessed by each task with five attributes. These five attributes are detailed in Section \ref{sec.realitybap}.


\subsection{Datasets}

In real-world scenarios, data is often collected using conservative policies. For most environments, we use the Soft Actor-Critic (SAC) algorithm \citep{sac2018} for online policy training to obtain high-performance policies. During training, we record the policy model after each round and rank them based on their performance. Considering that real-world methods are often non-optimal policies, we randomly select policies ranked within the 20-75\% range as sampling policies. In the DMSD environment, we employ the Bayesian Optimization parameter search method \citep{Fernando2014} to fine-tune the three key parameters of the PID controller. We rank all PIDs based on their performance and select the PID with a performance ranking of 56\% as the offline data sampling policy for the DMSD dataset.

After identifying the sampling policies, we collect data in all built-in environment simulators. \tzl{In most real-world tasks, there is typically only one policy for collecting offline datasets, leading to a lack of diversity. So, in NeoRL-2 it is important to clarify that all policies are deterministic when interacting with the environment to collect data.} The collected data are then divided into training and validation datasets, with 100,000 training dataset samples and 20,000 validation for each environment. Notably, the Fusion environment has a unique data sampling process due to the high cost of controlled nuclear fusion experiments. To reflect this, we limit the number of experimental trajectories, resulting in a training dataset of 2,000 samples and a validation dataset of 500 samples. Similarly, limited data availability is observed in the Rocket Recovery and Safety Halfcheetah environments, as detailed in Table \ref{task_configuration} of the Appendix \ref{sec.simulator}.

%In the real world, most tasks involve collecting data using a conservative strategy. Therefore, for most environments, we utilize the SAC \citep{sac2018} algorithm for online policy training with the objective of obtaining a high-performance policy. During the training process, we record the policy model after each round and rank them based on the performance of the policy in the environment. Due to the fact that sampling methods in real-world tasks are usually sub-optimal policies, we use policies ranked within the 20-75\% range as sampling policies. 

%What should be noted is that, in the DMSD environment, we employ the Bayesian Optimization parameter search method \citep{Fernando2014} to search for the three key parameters of the PID controller. Based on the search results, we rank all PIDs according to their performance. Finally, we select the PID with a performance ranking of 56\% as the offline data sampling policy for DMSD dataset.

%After obtaining the sampling policies, we perform data collection in all built-in environment simulators. The collected data is then divided into training and validation datasets. Specifically, for each environment, the offline data consists of 100,000 training samples.

%For the Fusion environment, the data sampling process is quite unique due to the high cost associated with conducting controlled nuclear fusion experiments in the real world. In order to better reflect this objective reality in our benchmark, we limited a very small number of experimental trajectories in the dataset. Therefore, we have further restricted the total amount of offline data for the Fusion environment. Specifically, the training data set consists of 2000 samples, while the validation dataset consists of 500 samples. Moreover, limited available data are also revealed in Rocket Recovery and Safety Half Cheetah as shown in Table \ref{task_configuration} of Appendix \ref{sec.simulator} 

==> sec_text/reality_gap.tex <==
\section{The Reality Gap}
\label{sec.realitybap}
\subsection{Motivation of NeoRL-2}
\tzl{Previously, the NeoRL benchmark only considered the fundamental data properties from real-world tasks, where the data was collected by a conservative policy with small noise and the size of datasets was limited. In our practice of offline RL after releasing NeoRL, we encountered more difficulties that were not reflected in NeoRL or other offline RL benchmarks. The problems we face in these scenarios can be categorized as {\bf time delay}, {\bf external factors}, {\bf policy constraints}, {\bf data collected based on traditional control methods}, and {\bf limitations on data} (even more constrained than those in NeoRL).}


\tzl{
Since the real world is open and real-world tasks are very complex, it is impossible that the 7 task scenarios in the NeoRL-2 benchmark can cover all the challenges. We intend to summarize the challenges in real-world settings and to create simulators that more accurately reflect these challenges, rather than providing a high-fidelity simulation environment. Thus, the most practical strategy is to reflect real-world issues as realistically as possible within the simulation environment. In addition, these properties indeed increase the difficulty of the task and lead to incomplete data. We hope that NeoRL-2 will encourage the community to pay more attention to these challenges when applying offline reinforcement learning to real-world tasks.
}


\subsection{Environment Properties}
The previously proposed benchmarks have played a significant role in advancing the development of offline RL techniques. However, based on our research, we have found notable gaps between real-world tasks and these benchmark tasks. Real-world tasks are generally more complex and challenging. Here, we articulate these properties that have been seen in real-world tasks but frequently neglected by those existing benchmarks:

\begin{enumerate}[itemsep=0pt,topsep=0pt,parsep=0pt,leftmargin=*]

\item \textbf{Delay:} Delay can be caused by various factors, including delays in sensor sampling, signal transmission delays, and response delays. It is ubiquitous in different tasks and increases the uncertainty and learning difficulty of a task, which induces a complex causality in understanding the system \citep{fridman2014introduction}. Delays can be observed not only in state transitions but also in obtaining rewards.

\item \textbf{External factors:} External factors are those that can affect the current system but are not influenced by the current internal system. Changes in these variables may modify the state distribution of the system environment, thus affecting the effectiveness of reward signals and policies \citep{2020Jinying}, further increasing the complexity and challenge of the task.

\item \textbf{Constrained control policies:} Real-world tasks often come with various constraints, which reveal physical limitations of the system, safety requirements, operational standards, or resource constraints \citep{2016Manuel}, where the datasets may only contain data that satisfies the constraint. Thus, due to the lack of exploration, offline algorithms can only learn from satisfactory data without explicitly knowing whether the current action will violate the constraint. 

\item \textbf{Data from traditional control methods:} In the real world, especially in the industrial sector, the control models in operation usually employ traditional control methods, such as PID. Data collected using these traditional methods tend to have a narrow distribution \citep{2022Tobias} and are difficult to be modeled. In addition, these traditional methods often rely on feedback control, which may lead to learning incorrect transition relationships.

\item \textbf{Limitations on data availability:} In many real-world tasks, obtaining a large amount of training data can not be practical, leading to the problem of data insufficiency. In some special scenarios, only a few trajectories of data can be ideally collected, which poses a significant challenge to the optimization of offline policies \citep{levine2020offline, Mandlekar2021}. We further reduce the amount of datasets to match the real-world scenarios.

\end{enumerate}

Therefore, we propose NeoRL-2 as a supplement and improvement to existing benchmarks. The tasks in NeoRL-2 cover a wider range of real-world applications, including time-delay environmental transitions, external influencing factors, global constraints, data collected from traditional control methods, and limited data availability.

\tzl{Factors such as delays, external influences, constrained control policies, and data derived from traditional control methods significantly increase the task complexity and lead to data incompleteness. For instance, a large delay makes the action effect last an indefinitely long period, making the control policy non-Markovian. Policy constraints often restrict the data collection to only safe states and actions, resulting in incomplete space coverage. Additionally, external factors can introduce variability and may not be explicitly reflected in the dataset. All of these factors directly lead to the incompleteness of the observed information, gradually deviating from the standard MDP/POMDP assumptions. As many current offline reinforcement learning algorithms overlook these issues, these challenges could pose significant difficulties.}


==> sec_text/related_work.tex <==
\section{Related Work}

\subsection{Offline RL}

Offline RL focuses on learning from historical datasets. Unlike traditional online RL, offline RL does not require iterative interactions with the environment to update the policy. This requires algorithms to be capable of handling issues such as distributional shift \citep{2019Aviral} in the data, sparse rewards \citep{2022RengarajanVSKS}, and potential non-Markovian \citep{lauri2023survey} behavior.

Compared to online RL, a key advantage of offline RL is the ability to leverage existing historical data, which is highly valuable in many practical applications such as healthcare \citep{2006Damien,2017Niranjani,2018Komorowski}, industrial settings\citep{DENG2023221}, robotics\citep{2021Yevgen}, and autonomous driving \citep{2022Kiran}. In these domains, interacting with the environment is highly cost, risky, or impractical. Through offline RL, it is possible to learn and extract optimized policies from existing data without the need for additional online data collection.

Offline RL methods typically include model-free approaches and model-based approaches. Model-free methods directly learn policies or value functions from data without attempting to construct a dynamic model of the environment \citep{2018Sutton}. This includes techniques such as $Q$-learning and policy gradients. Model-based methods often start by learning a dynamics model of the environment from offline data and then use these models for planning or policy improvement through simulation \citep{luo2024survey}.

To address the challenges of offline RL, researchers have proposed various methods, primarily including policy constraint methods. These approaches minimize the impact of distributional shift by constraining the differences between the learning policy and the behavior policy \citep{workflow_offline_cql.2021, 2021td3bc}. For instance, they penalize actions that deviate from the original data distribution to prevent overestimation issues during the policy learning process \citep{yu2020mopo}. There are also methods based on uncertainty: These leverage the uncertainty inherent in the data to guide policy learning, balancing exploration and exploitation by estimating the uncertainty of the value function or the policy itself \citep{2023filter}. Regularization methods for the value function are another approach: These reduce the deviation of the learning policy from the original data distribution by incorporating regularization terms into the optimization process of the value function \citep{2021edac}. These methods aim to address key issues in offline RL, such as data quality, and distributional shift issues. 

% In summary, offline reinforcement learning is an active research field that provides a way to learn effective policies from historical data without environment interaction. With technological advancements, offline reinforcement learning has the potential to play an important role in many practical problems, particularly in scenarios where the cost or feasibility of online data collection is high.

\subsection{Offline RL Algorithm Benchmark}

Offline RL benchmarks play a crucial role in evaluating algorithms and advancements in the field by offering standardized environments and datasets \citep{levine2020offline}. Three notable benchmarks for testing and enhancing offline RL methods are D4RL \citep{D4RL}, RL Unplugged \citep{RLunplugged}, and NeoRL \citep{qinr2022neorl}, each with its unique focuses and dataset characteristics. 

D4RL is designed to mirror real-world challenges using datasets generated from various policies, including hand-designed controllers and human demonstrators. It covers properties like narrow and biased data distributions, sparse rewards, and sub-optimal data, facilitating existing offline algorithms and exposing potential flaws not evident in simpler tasks or datasets.
RL Unplugged provides a suite of datasets from domains such as games (e.g., Atari) and simulated motion control problems (e.g., DeepMind Control Suite). Emphasizing learning from offline datasets, it aims to overcome challenges like cost, safety, and ethical issues associated with online data collection. It provides clear evaluation protocols and reference performance baselines, facilitating researchers in comparing and analyzing different offline RL methods effectively. NeoRL focuses on the nature of datasets from real-world scenarios. It emphasizes conservative actions, limited data, and offline policy evaluation. By doing so, it aims to facilitate the development of offline RL algorithms better suited for real-world applications and promote the adoption of offline policy evaluation methods for improved policy selection before real-world deployment.

%Offline RL benchmarks play a crucial role in evaluating algorithms and driving the advancement of the field by providing standardized environments and datasets \citep{levine2020offline}. Three notable benchmarks for testing and improving offline RL methods are D4RL~\citep{D4RL, 2021justin}, RL Unplugged \citep{RLunplugged} and NeoRL \citep{2022qin}, each with unique focus and dataset characteristics.

%D4RL focuses on creating a benchmark that better reflects real-world challenges, including datasets generated from various policies such as hand-designed controllers, human demonstrators, and different policy combinations. D4RL tasks cover varied properties that may be encountered in practical applications, including narrow and biased data distributions, uni-modal and multitask data, sparse rewards, and sub-optimal data. The benchmark aims to push the boundaries of existing algorithms and reveal defects that may not be apparent in simpler tasks or datasets.

%RL Unplugged is a benchmark suite that focuses on bridging the gap between RL research and real-world applications by providing various datasets from domains such as games (e.g., Atari) and simulated motion control problems (e.g., DeepMind Control Suite). The benchmark emphasizes the importance of learning from offline datasets to overcome challenges associated with online data collection, such as cost, safety, and ethical issues. RL Unplugged provides clear evaluation protocols and reference performance baselines for the datasets, making it easier for researchers to compare and analyze the performance of different offline RL methods.

%NeoRL provides a benchmark for offline RL that approaches real-world scenarios and addresses gaps of the real world present in existing benchmarks. 
%NeoRL emphasizes the importance of conservative actions, limited data, stochastic dynamics, and offline policy evaluation, which are common and critical factors in real-world decision-making scenarios. The benchmark aims to facilitate the design of offline RL algorithms that are better suited for real-world applications and promote the use of offline policy evaluation methods for better policy selection before practicing in the real world.
